On the Sequential Probability Ratio Test in Hidden Markov Models

We consider the Sequential Probability Ratio Test applied to Hidden Markov Models. Given two Hidden Markov Models and a sequence of observations generated by one of them, the Sequential Probability Ratio Test attempts to decide which model produced the sequence. We show relationships between the execution time of such an algorithm and Lyapunov exponents of random matrix systems. Further, we give complexity results about the execution time taken by the Sequential Probability Ratio Test.

==> difffile <==
Index: lyapunovhmm.tex
===================================================================
--- lyapunovhmm.tex	(revision 269)
+++ lyapunovhmm.tex	(revision 294)
@@ -11,6 +11,7 @@
 \tikzset{LMC style/.style={>=angle 60,every edge/.append style={thick},every state/.style={thick,minimum size=20,inner sep=0.5}}}
 
 \usepackage{asymptote}
+\usepackage{pgfplots, pgfplotstable}
 
 \newcommand{\eow}{\$}
 \newcommand{\RR}{\mathbb{R}}
@@ -233,16 +234,16 @@
 $[d] = \{1, \dots, d\}$. % and $[Q] = \{1, \dots, |Q|\}$.
 For a finite set~$Q$, vectors $\mu \in \RR^Q$ are viewed as row vectors, and their transpose (a column vector) is denoted by $\mu^\top$.
 The norm $\|\mu\|$ is assumed to be the $l_1$ norm: $\| \mu \| = \sum_{q \in Q} | \mu_q |$.
-We write $\vec{0}, \vec{1}$ for the vectors all whose entries are $0$, $1$, respectively.
+We write $\vec{0}, \vec{1}$ for the vectors all of whose entries are $0$, $1$, respectively.
 For $q \in Q$, we denote by~$e_q \in \{0,1\}^Q$ the vector with $(e_q)_q = 1$ and $(e_q)_{q'} = 0$ for $q' \ne q$.
 A matrix $M \in [0,1]^{Q \times Q}$ is \emph{stochastic} if $\vec{1}^\top = M \vec{1}^\top$.
 We often identify vectors $\mu \in [0,1]^Q$ such that $\| \mu \| = 1$ with the corresponding probability distribution on~$Q$.
 For $\mu \in [0,\infty)^Q$ we write $\supp(\mu) := \{q \in Q \mid \mu_q > 0\}$.
 
-For a finite alphabet~$\Sigma$ and $n \in \NN$ we denote by $\Sigma^n, \Sigma^*, \Sigma^\omega$ the sets of length-$n$ words, finite words, infinite words, respectively.
+For a finite alphabet~$\Sigma$ and $n \in \NN$ we denote by $\Sigma^n, \Sigma^*, \Sigma^+, \Sigma^\omega$ the sets of length-$n$ words, finite words, non-empty finite words, infinite words, respectively.
 For $w \in \Sigma^\omega$ we write $w_n$ for the length-$n$ prefix of~$w$.
 
-A \emph{Hidden Markov Model} (HMM) is a triple $\H = (Q, \Sigma, \Psi)$ where $Q$ is a finite set of states, $\Sigma$ is a set of observations (or ``letters''), and the function $\Psi : \Sigma \rightarrow [0,1]^{Q \times Q}$ specifies the transitions such that $\sum_{a \in \Sigma} \Psi(a)$ is stochastic.
+A \emph{Hidden Markov Model} (HMM) is a triple $\H = (Q, \Sigma, \Psi)$ where $Q$ is a finite set of states, $\Sigma$ is a set of observations (or ``letters''), and the function $\Psi : \Sigma \rightarrow [0,1]^{Q \times Q}$ specifies the transitions such that $\sum_{a \in \Sigma} \Psi(a)$ is stochastic. For computational purposes we assume the numbers in $\Psi$ are rational and expressed as fractions of integers encoded in binary.
 A \emph{Markov chain} is a pair $(Q, T)$ where $Q$ is a finite set of states and $T \in [0,1]^{Q \times Q}$ is a stochastic matrix.
 A Markov chain $(Q,T)$ is naturally associated with its directed \emph{graph} $(Q,\{(q,r) \mid T_{q,r} > 0\})$, and so we may use graph concepts, such as strongly connected components (SCCs), in the context of a Markov chain. Trivial SCCs are considered SCCs.
 The \emph{embedded} Markov chain of an HMM $(Q, \Sigma, \Psi)$ is the Markov chain $(Q, \sum_{a \in \Sigma} \Psi(a))$.
@@ -255,7 +256,7 @@
 Fix an HMM $\H = (Q, \Sigma, \Psi)$ for the rest of the section.
 We extend $\Psi$ to the mapping $\Psi : \Sigma^* \rightarrow [0,1]^{Q \times Q}$ with $\Psi(a_1 \cdots a_n) = \Psi(a_1) \cdot \ldots \cdot \Psi(a_n)$ and $\Psi(\epsilon) = I$, where $\epsilon$ is the empty word and $I$ the $Q \times Q$ identity matrix.
 We call a finite sequence $v = q_0 a_1 q_1 \cdots a_n q_n \in Q (\Sigma Q)^*$ a \emph{path} and $v (\Sigma Q)^\omega$ a \emph{cylinder set} and an infinite sequence $q_0 a_1 q_1 a_2 q_2 \cdots \in Q (\Sigma Q)^\omega$ a \emph{run}.
-To~$\H$ and an \emph{initial probability distribution} $\pi \in [0,1]^Q$ we associate the probability space $(Q(\Sigma Q)^\omega, \GG^*, \PP_\pi)$ where $\GG^*$ is the $\sigma$-algebra generated by the cylinder sets and $\PP_\pi$ is the unique probability measure with $\PP_\pi(q_0 a_1 q_1 \cdots a_n q_n (\Sigma Q)^\omega) = \pi_q \prod_{i=1}^{n} \Psi(a_i)_{q_{i-1},q_i}$.
+To~$\H$ and an \emph{initial probability distribution} $\pi \in [0,1]^Q$ we associate the probability space $(Q(\Sigma Q)^\omega, \GG^*, \PP_\pi)$ where $\GG^*$ is the $\sigma$-algebra generated by the cylinder sets and $\PP_\pi$ is the unique probability measure with $\PP_\pi(q_0 a_1 q_1 \cdots a_n q_n (\Sigma Q)^\omega) = \pi_{q_0} \prod_{i=1}^{n} \Psi(a_i)_{q_{i-1},q_i}$.
 As the states are often irrelevant, for $E \subseteq \Sigma^\omega$ and $\uparr{E} := \{q_0 a_1 q_1 a_2 q_2 \cdots \mid a_1 a_2 \cdots \in E\} \in \GG^*$ we view also $E$ as an event and may write $\PP_{\pi}(E)$ to mean $\PP_{\pi}(\uparr{E})$.
 In particular, for $w \in \Sigma^*$ we have $\PP_{\pi}(w \Sigma^\omega) = \| \pi \Psi(w) \|$.
 For $E \subseteq \Sigma^\omega$ we write $\1_E$ for the indicator random variable with $\1_E(w) = 1$ if $w \in E$ and $\1_E(w) = 0$ if $w \not\in E$.
@@ -418,7 +419,7 @@
 The following theorem is perhaps the most fundamental contribution of this paper.
 \begin{restatable}{theorem}{liexplimits}\label{liexplimits}
 For any initial distributions $\pi_1, \pi_2$ the limit $\liexp$ exists $\PP_{\pi_2}$-almost surely.
-Furthermore, we have $|\Lambda| \le |Q|^2+1$.
+Furthermore, we have $|\Lambda | \leq |Q|^2+1$.	
 %The set of likelihood exponents satisfies $\Lambda \subset [-\infty, 0]$ and $|\Lambda| \leq |Q|^2$. Further $\liexp$ exists (and by definition is in $\Lambda$) $\PP_{\pi_2}$-almost surely for any $\pi_1, \pi_2$.
 \end{restatable}
 It follows from a stronger theorem, \cref{thm:likelihood-to-lyapunov}, which we prove in \cref{sec:rep}.
@@ -556,9 +557,9 @@
 \begin{restatable}{theorem}{thmqualprob} \label{thm:qual-prob}
 Given an HMM and initial distributions $\pi_1, \pi_2$,
 \begin{enumerate}
-\item one can compute $\PP_{\pi_2}(E_{-\infty})$ and $\PP_{\pi_2}(E_0)$ in PSPACE;
-\item one can decide whether $\PP_{\pi_2}(E_0)=0$ (i.e., $0 \not\in \Lambda_{\pi_1,\pi_2}$) in polynomial time;
-\item deciding whether $\PP_{\pi_2}(E_0)=1$, whether $\PP_{\pi_2}(E_{-\infty})=0$, and whether $\PP_{\pi_2}(E_{-\infty})=1$ are all PSPACE-complete problems.
+\item one can compute $\PP_{\pi_2}(\liexp = -\infty)$ and $\PP_{\pi_2}(\liexp = 0)$ in PSPACE;
+\item one can decide whether $\PP_{\pi_2}(\liexp  =0)=0$ (i.e., $0 \not\in \Lambda_{\pi_1,\pi_2}$) in polynomial time;
+\item deciding whether $\PP_{\pi_2}(\liexp = 0)=1$, whether $\PP_{\pi_2}(\liexp = -\infty)=0$, and whether $\PP_{\pi_2}(\liexp  = -\infty)=1$ are all PSPACE-complete problems.
 \end{enumerate}
 \end{restatable}
 
@@ -710,14 +711,14 @@
 
 %Let $((Q, \Sigma, \Psi), \rho)$ be a Lyapunov system.
 We can identify the probability distribution $\rho$ from this definition with the single-state HMM $(\{s\}, \Sigma, \Psi_\rho)$ where $\Psi_\rho(a)_{s,s} = \rho(a)$ for all $a \in \Sigma$.
-In this way, $\rho$ produces a random infinite word from $\Sigma^\omega$.
-The following lemma is known from~\cite{prot13}.
+In this way, $\rho$ produces a random infinite word from $\Sigma^\omega$. We will write $\PP_{\rho} $ for the associated probability measure.
+The following lemma is Theorem 1 from~\cite{prot13}.
 
 \begin{lemma}[\cite{prot13}] \label{lem:lyapunov-exponent}
 Let $((Q, \Sigma, \Psi), \rho)$ be a Lyapunov system.
-Then there is $\lambda \in \RR$ such that, for all $q \in Q$, $\PP_{\rho}$-a.s., either $e_q \Psi(w_n) = \vec{0}$ for some $n \in \NN$ or the limit $\lim_{n \to \infty} \frac1n \ln \| e_q \Psi(w_n) \|$ exists and equals~$\lambda$.
+Then there is $\lambda \in \RR$ such that, for all $\pi \in [0,\infty)^Q$, $\PP_{\rho}$-a.s., either $\pi \Psi(w_n) = \vec{0}$ for some $n \in \NN$ or the limit $\lim_{n \to \infty} \frac1n \ln \| \pi \Psi(w_n) \|$ exists and equals~$\lambda$.
 \end{lemma}
-For a Lyapunov system~$\S$ we call $\lambda(\S) = \lambda$ from the lemma the \emph{Lyapunov exponent} defined by~$\S$.
+For a Lyapunov system~$\S$ we call $\lambda(\S) = \lambda$ from the lemma the \emph{Lyapunov exponent} defined by~$\S$. In the case that $\PP_{\pi_2}$-a.s. for all $\pi \in [0,1]^Q$ there is $n \in \NN$ such that $ \Psi(w_n) = \vec{0}$ we say $\lambda(\S) = -\infty$.
 We prove the following theorem, which implies \cref{liexplimits}.
 \begin{restatable}{theorem}{likelihoodtolyapunov}\label{thm:likelihood-to-lyapunov}
 Given an HMM $(Q, \Sigma, \Psi)$ we can compute in polynomial time $2 K \le 2 |Q|^2$ Lyapunov systems $\S_1^1, \S_1^2, \S_2^1, \S_2^2, \ldots, \S_K^1, \S_K^2$ such that for any initial distributions $\pi_1, \pi_2$ the limit $\liexp$ exists $\PP_{\pi_2}$-a.s.\ and lies in
@@ -730,11 +731,12 @@
 
 In the rest of the section we provide more details on the construction underlying \cref{thm:likelihood-to-lyapunov}.
 As an intermediate concept (between the given HMM and the Lyapunov systems from \cref{thm:likelihood-to-lyapunov}) we define \emph{generalized Lyapunov systems}.
-
+\def\generalizedlyapsysdef{
 First, for two matrix systems $\M_1 = (Q_1,\Sigma,\Psi_1)$ and $\M_2 = (Q_2,\Sigma,\Psi_2)$ with finite $Q_1, Q_2, \Sigma$ and transitions $\Psi_1,\Psi_2 : \Sigma \to \RR_{\ge 0}^{Q \times Q}$ we define the directed graph $G_{\M_1,\M_2} = (Q_1 \times Q_2, E)$ such that there is an edge from $(q_1,q_2)$ to $(r_1,r_2)$ if there is $a \in \Sigma$ with $\Psi_1(a)_{q_1,r_1} > 0$ and $\Psi_2(a)_{q_2,r_2} > 0$.
 
 A \emph{generalized Lyapunov system} is a triple $\S = (\M,\H,C)$ where $\M = (Q_1, \Sigma, \Psi_1)$ is a matrix system and $\H = (Q_2, \Sigma, \Psi_2)$ is a strongly connected HMM and $C \subseteq Q_1 \times Q_2$ is a bottom SCC of $G_{\M, \H}$.
 Given a generalized Lyapunov system, one can efficiently compute an ``equivalent'' Lyapunov system:
+}
 \begin{restatable}{lemma}{fromgentonongen}\label{from-gen-to-nongen}
 Let $\S = ((Q_1, \Sigma, \Psi_1),(Q_2, \Sigma, \Psi_2),C)$ be a generalized Lyapunov system.
 \begin{enumerate}
@@ -745,6 +747,7 @@
 \end{enumerate}
 \end{restatable}
 
+\def\definitionsforgenlyap{
 Let $\H = (Q,\Sigma,\Psi)$ be an HMM.
 Let $R \subseteq Q \times Q$ be a (not necessarily bottom) SCC of the graph $G_{\H,\H}$ such that $Q_R := \{q_2 \in Q \mid \exists\,q_1 \in Q : (q_1,q_2) \in R\}$ is a bottom SCC of the graph of $\sum_{a \in \Sigma} \Psi(a)$.
 We call such~$R$ a \emph{right-bottom} SCC.
@@ -773,6 +776,10 @@
 and $C^2 := \{((q_1,q_2),q_2) \mid (q_1,q_2) \in R'\}$.
 
 For sets $U, V \subseteq Q \times Q$ let $U \longrightarrow_{G_{\H,\H}} V$ denote that there are $u \in U$ and $v \in V$ such that $v$ is reachable from~$u$ in~$G_{\H,\H}$.
+}
+
+\definitionsforgenlyap
+
 We are ready to state the following key technical lemma:%
 %\begin{lemma} \label{lem:construct-L-systems}
 %Given an HMM $(Q, \Sigma, \Psi)$, let $\mathcal{R} \subseteq 2^{Q \times Q}$ be the set of its right-bottom SCCs, and, for $R \in \mathcal{R}$, let $\S_{R}^1, \S_{R}^2$ be the generalized Lyapunov systems defined above.
@@ -1105,7 +1112,7 @@
 \end{lemma}
 
 \begin{proof}[Proof of \Cref{probexp0}]
-By \cref{lem:expoprop} there are a set of bottom SCCs $\mathcal{Z}$ in $\mathcal{B}$. Such that for all $Z \in \mathcal{Z}$ we have $\ell(Z) = \{0\}$. Let $\pi \in [0,1]^Q$ and $r \in Q$ such that $(\supp~\pi, r) \in Z$. Suppose that $\pi$ and $\delta_r$ are distinguishable then by \Cref{kief16thm5} both $\PP_{\delta_r}(L_n^* \geq 1) \leq 2\exp\big( -\frac{c^2}{18}n \big)$ and $\PP_{\pi}(L_n^* \leq 1) \leq 2\exp\big( -\frac{c^2}{18}n \big)$ where $L_n^*$ is the likelihood ratio started from initial distributions $\pi$ and $\delta_r$. Fix $-\frac{c^2}{18} \leq \alpha \leq 0$ and define the event $W_n = \{1 > L_n^* \geq \e^{n\alpha}\}$. Then
+By \cref{lem:expoprop} there are a set of bottom SCCs $\mathcal{Z}$ in $\mathcal{B}$. Such that for all $Z \in \mathcal{Z}$ we have $\ell(Z) = \{0\}$. Let $\pi \in [0,1]^Q$ and $r \in Q$ such that $(\supp~\pi, r) \in Z$. Suppose that $\pi$ and $\delta_r$ are distinguishable then by \Cref{kief16thm5} both $\PP_{\delta_r}(L_n^* \geq 1) \leq 2\exp\big( -\frac{c^2}{18}n \big)$ and $\PP_{\pi}(L_n^* \leq 1) \leq 2\exp\big( -\frac{c^2}{18}n \big)$ where $L_n^*$ is the likelihood ratio started from initial distributions $\pi$ and $\delta_r$. Fix $-\frac{c^2}{18} < \alpha \leq 0$ and define the event $W_n = \{1 > L_n^* \geq \e^{n\alpha}\}$. Then
 \begin{align*}
 \PP_{\delta_r}(\lim_{n \rightarrow \infty} \frac1n \ln L_n^* > \alpha) & \leq \PP_{\delta_r}(\liminf_n \{\frac1n \ln L_n^* \geq \alpha\}) \\
 & \leq \liminf_n \PP_{\delta_r}(\frac1n \ln L_n^* \geq \alpha) \\
@@ -1114,7 +1121,7 @@
 & \leq \liminf_n \Big[ \sum_{w \in W_n} \delta_r \Psi(w) \1^T + 2\exp\big( -\frac{c^2}{18}n \big) \Big]\\
 & \leq \liminf_n \Big[ e^{-n\alpha} \sum_{w \in W_n} \pi \Psi(w) \1^T\Big]\\
 & \leq \liminf_n \Big[ e^{-n\alpha} \PP_{\pi}(L_n^* < 1)\Big]\\
-& \leq \liminf_n \Big[ e^{-n\alpha} 2\exp\big( -\frac{c^2}{18}n \big)\Big]\\
+& \leq \liminf_n \Big[ 2e^{-n\alpha} \exp\big( -\frac{c^2}{18}n \big)\Big]\\
 & = 0.
 \end{align*}
 In particular, $\PP_{\pi_2}(\lim_{n \rightarrow \infty} \frac1n \ln L_n = 0 ) = 0$ which contradicts $\Lambda = \{0\}$. Hence $\pi$ and $\delta_r$ are not distinguishable and so $\PP_{\delta_r}$-almost surely, we have $\lim_{n \rightarrow \infty} L_n^* > 0$. By conditioning on the events $\{a_1 r_1 \cdots a_n r_n \in (\Sigma Q)^* \mid \supp~\pi_1 \Psi(w) = \supp~ \pi, r_n = r\}$ it follows that $E_0 = \{\lim_{n \rightarrow \infty} L_n > 0\}$. We now show the second equality. If $\lim_{n \rightarrow \infty} L_n > 0$ then for $\alpha, \beta$ small enough $L_n$ never crosses the SPRT bounds. Hence, we have $\{\lim_{n \rightarrow \infty} L_n > 0\} \subseteq \bigcup_{\alpha, \beta} \{N_{\alpha, \beta} = \infty\}$. For the converse inclusion, suppose that $N_{\alpha, \beta} = \infty$ for some $\alpha, \beta$ this would contradict $\lim_{n \rightarrow \infty} L_n = 0$ since then $N_{\alpha, \beta}$ would be $\PP_{\pi_2}$-almost surely finite.
@@ -1162,11 +1169,11 @@
 \end{lemma}
 
 \begin{proof}[Proof of \Cref{unifintegofN}]
-By \Cref{liexpmotivation}, conditioned on $E_\ell$ we have $\lim_{\alpha, \beta \rightarrow 0} \frac{N_{\alpha, \beta}}{\ln \alpha}$ exists $\PP_{\pi_2}$-almost surely. Hence, the convergence is also in $\PP_{\pi_2}$-measure. Therefore, by the Vitali convergence theorem\cite{bog2007} it is sufficient to show that the set of random variables $\{ \frac{N_{\alpha, \beta}}{\ln \alpha} \mid \alpha, \beta \in (0,\frac12) \}$ is uniformly integrable conditioned on $V_k$. In fact, because
+By \Cref{liexpmotivation}, conditioned on $E_\ell$ we have $\lim_{\alpha, \beta \rightarrow 0} \frac{N_{\alpha, \beta}}{\ln \alpha}$ exists $\PP_{\pi_2}$-almost surely. Hence, the convergence is also in $\PP_{\pi_2}$-measure. Therefore, by the Vitali convergence theorem \cite{bog2007} it is sufficient to show that the set of random variables $\{ \frac{N_{\alpha, \beta}}{\ln \alpha} \mid \alpha, \beta \in (0,\frac12) \}$ is uniformly integrable conditioned on $E_\ell$. In fact, because
 \begin{equation}\label{unifintcond}
 \lim_{K \rightarrow \infty} \sup_{\alpha, \beta} \EE_{\pi_2} \big[ \frac{N_{\alpha, \beta}}{- \ln \alpha}\1_{\frac{N_{\alpha, \beta}}{-\ln \alpha} \geq - K}\big] \geq \PP_{\pi_2}(E_\ell) \lim_{M \rightarrow \infty} \sup_{\alpha, \beta} \frac{1}{- \ln \alpha}\EE_{\pi_2} \big[ \frac{N_{\alpha, \beta}}{- \ln \alpha}\1_{\frac{N_{\alpha, \beta}}{-\ln \alpha} \geq - K} \mid E_\ell \big],
 \end{equation}
-It is sufficient to check the uniform integrability condition without conditioning on $V_k$.
+It is sufficient to check the uniform integrability condition without conditioning on $E_\ell$.
 
 For fixed $M \geq \frac{144|Q|}{c^2}$, write $m_\alpha = \floor{\frac{- M \ln \alpha}{2|Q|}}$. It follows that 
 \begin{equation*}
@@ -1184,7 +1191,7 @@
 & \leq 4M \exp{-\frac{c^2}{36} \Big(\frac{M \ln 2}{2|Q|} - 1 \Big)}  + \frac{8|Q|\exp \Big( -\frac{c^2}{36} (\frac{M \ln 2}{2|Q|} - 1 ) \Big) }{\ln 2} \frac{1}{1 - \exp{c^2 / 36}}\\
 & \rightarrow 0
 \end{align*}
-as $K \rightarrow \infty$ where the fourth inequality follows by \Cref{2016profilethm}. Hence, \Cref{unifintcond} must hold.
+as $M \rightarrow \infty$ where the fourth inequality follows by \Cref{2016profilethm}. Hence, \Cref{unifintcond} must hold.
 \end{proof}
 
 \liexpmotivation*
@@ -1194,7 +1201,7 @@
 \begin{equation*}
 N_{\alpha,\beta} \geq \frac{ \min \{ \ln \frac{\alpha}{1 - \beta}, \ln \frac{\beta}{1 - \alpha} \} }{\ln \Psimin}
 \end{equation*}
-Hence $N_{\alpha, \beta} \rightarrow \infty \ \PP_{\pi_2}$-almost surely as $\alpha, \beta \rightarrow 0$. Consider the case $\ell_k \in (-\infty, 0)$. Let $U_{\alpha,\beta} = \{w \in \Sigma^\omega \mid \ln L_{N_\alpha} \leq \ln \frac{ \alpha}{1 - \beta} \}$. The set $\bigcap_{\alpha, \beta \in (0,1]} U_{\alpha, \beta}^c \subseteq \{L_n \text{ is unbounded}\}$. Hence, $\lim_{\alpha, \beta \rightarrow 0}\1_{U_{\alpha,\beta}} = 1 \ ~\PP_{\pi_2}$-almost surely. Conditioned on $V_k$ it follows that
+Hence $N_{\alpha, \beta} \rightarrow \infty \ \PP_{\pi_2}$-almost surely as $\alpha, \beta \rightarrow 0$. Consider the case $\ell_k \in (-\infty, 0)$. Let $U_{\alpha,\beta} = \{w \in \Sigma^\omega \mid \ln L_{N_\alpha} \leq \ln \frac{ \alpha}{1 - \beta} \}$. The set $\bigcap_{\alpha, \beta \in (0,1]} U_{\alpha, \beta}^c \subseteq \{L_n \text{ is unbounded}\}$. Hence, $\lim_{\alpha, \beta \rightarrow 0}\1_{U_{\alpha,\beta}} = 1 \ ~\PP_{\pi_2}$-almost surely. Conditioned on $E_\ell$ it follows that
 
 \begin{equation*}
 0 \leq \1_{U_{\alpha, \beta}} \frac{\ln \frac{\alpha}{1 - \beta} - \ln L_{N_{\alpha, \beta}}}{N_\alpha} \leq \1_{U_{\alpha, \beta}}  \frac{\ln L_{N_{\alpha, \beta} - 1}  - \ln L_{N_{\alpha, \beta}}}{N_{\alpha, \beta}}\rightarrow 0 \ \text{ as } \alpha \rightarrow 0.
@@ -1407,163 +1414,381 @@
 
 \section{Proofs from \Cref{sec:rep}}
 
+For ease of reading, we repeat some definitions from \Cref{sec:rep}.
+
+\generalizedlyapsysdef
+
 \fromgentonongen*
+The following is the key technical lemma that we use to prove \Cref{from-gen-to-nongen}. 
 
+\begin{lemma}\label{makereduciblelyapsys}
+	Let $\mathcal{H} = (Q, \Sigma, \Psi)$ be an HMM and define $\Psi'$ as in the main text such that $\mathcal{H}' = (Q, \Sigma Q, \Psi')$ is an HMM. One can compute in polynomial time a finite set $\Delta$, a probability distribution $\rho \in (0,1]^{\Delta}$ and for each $r_0 \in Q$ (a representation of) a mapping $\kappa_{r_0} : \Delta \rightarrow (\Sigma Q)$ with the following property. 
+	
+	Extend $\kappa_{r_0}$ to $(\Sigma Q)^+$ inductively. For each $c \in \Delta$ and $\overline{w} \in \Delta^+$ we let $\kappa_{r_0}(c~\overline{w}) = (a_1 r_1) \kappa_{r_1}(\overline{w})$ where $a_1 r_1 = \kappa_{r_0}(c)$. Then, for each word $w \in (\Sigma Q)^+$ we have
+	\begin{equation}\label{markov2indepmeasures}
+	\PP_{\rho}(\kappa_{r_0}^{-1}(\{w\}) \Delta^\omega) = \PP_{e_{r_0}}(w (\Sigma Q)^\omega)
+	\end{equation}
+	where $\PP_{e_{r_0}}$ refers to the measure on words produced by $\mathcal{H}'$ with initial distribution $e_{r_0}$.
+\end{lemma}
+
 \begin{proof}
-Since for each $p \in Q_2$, $\sum_{a \in \Sigma} \sum_{q \in Q_2} \Psi_2(a)_{p,q} = 1$ it follows that we may define a function $\kappa_p : [0,1) \rightarrow Q_2 \times \Sigma$ such that for all $p \in Q_2$, The Lebesgue measure $\MLeb(\kappa_p^{-1}\{(q, a)\}) = \Psi(a)_{p,q}$.
-Let $\Sigma'$ be the set of atomic elements of the finite $\sigma$-algebra $\sigma\{\kappa_p^{-1}\{(q, a)\} \mid p,q \in Q_2, a \in \Sigma\}$. Let $Q' = C$. We also define the transition matrix $\Psi : \Sigma' \rightarrow \RR_{\geq 0}^{C \times C}$
+	Let $\tau : [\Sigma Q] \rightarrow \Sigma Q$ be a bijection which we view as an arbitrary ordering on $\Sigma Q$ and write $\tau(k) = a_k q_k$. For each $r \in Q$ we define a function $\overline{\kappa}_r: [0,1) \rightarrow \Sigma Q$
+	\begin{equation*}
+	\overline{\kappa}_r(x) = a_K q_K \text{ when } \sum_{k = 1}^{K - 1} \Psi(a_k)_{r, q_k} \leq x < \sum_{k = 1}^K \Psi(a_k)_{r, q_k},
+	\end{equation*}
+	where for notational purposes, $\sum_{k = 1}^{0} \Psi(a_k)_{p, q_k} = 0$. For each $r \in Q$, since $\sum_{k = 1}^{|Q \times \Sigma|} \Psi(a_k)_{r, q_k} = 1$ it follows that $\overline{\kappa}_r$ is well defined on the interval $[0,1)$. Let $\Delta$ be the set of atomic elements of the finite $\sigma$-algebra $\sigma\{\overline{\kappa}_r^{-1}(\{a q\}) \mid r,q \in Q, a \in \Sigma\}$. The set $\Delta$ is a finite partition of $[0,1)$ and consists of intervals $[\alpha, \beta)$ where $\alpha, \beta \in [0,1]\cap\QQ$. We demonstrate the construction of $\Delta$ using the example HMM below.
+	
+	\begin{center}
+		\begin{tikzpicture}[scale=2.5,LMC style]
+		\node[state] (q1) at (-1,0) {$q_1$};
+		\node[state] (q2) at (0,0) {$q_2$};
+		\node[state] (q3) at (1,0) {$q_3$};
+		
+		\path[->] (q1) edge [loop,out=140,in=100,looseness=10] node[left] {$0.2 a$} (q1);
+		\path[->] (q1) edge [loop,out=260,in=220,looseness=10] node[left] {$0.4 b$} (q1);
+		\path[->] (q1) edge [bend left] node[above] {$0.4 b$} (q2);
+		
+		
+		\path[->] (q2) edge [loop,out=110,in=70,looseness=10] node[above] {$0.4 a$} (q2);
+		\path[->] (q2) edge [bend left] node[below] {$0.3 b$} (q1);
+		\path[->] (q2) edge [bend left] node[above] {$0.3 b$} (q3);
+		
+		\path[->] (q3) edge [loop,out=80,in=40,looseness=10] node[right] {$0.6 a$} (q3);
+		\path[->] (q3) edge [loop,out=-40,in=-80,looseness=10] node[right] {$0.2 b$} (q3);
+		\path[->] (q3) edge [bend left] node[above] {$0.2 b$} (q2);
+		\end{tikzpicture}
+	\end{center}
+	In the diagram below we give a representation of the functions $\overline{\kappa}_{q_1}, \overline{\kappa}_{q_2}, \overline{\kappa}_{q_3}$ and also the resulting set $\Delta$. The first three horizontal stacks of rectangles each represent a partition of the interval $[0,1)$ into the values taken by $\overline{\kappa}_{q_i}$ for $i = 1, 2, 3$. The bottom horizontal stack of rectangles represent the intervals in $\Delta$.
+	\begin{center}
+		\begin{tikzpicture}
+		\draw[black, very thick] (0,-1.25) rectangle (2.2,-1.75);
+		\draw[black, very thick] (2.2,-1.25) rectangle (4.4,-1.75);
+		\draw[black, very thick] (4.4,-1.25) rectangle (6.6,-1.75);
+		\draw[black, very thick] (6.6,-1.25) rectangle (7.7,-1.75);
+		\draw[black, very thick] (7.7,-1.25) rectangle (8.8,-1.75);
+		\draw[black, very thick] (8.8,-1.25) rectangle (11,-1.75);
+		\node[] at (0,-1) {$0$};
+		\node[] at (2.2,-1) {$0.2$};
+		\node[] at (4.4,-1) {$0.4$};
+		\node[] at (6.6,-1) {$0.6$};
+		\node[] at (7.7,-1) {$0.7$};
+		\node[] at (8.8,-1) {$0.8$};
+		\node[] at (11,-1) {$1$};
+		
+		\node[] at (-0.5,-1.5) {$\Delta$};
+		
+		\draw [-latex](5.5,-0.25) -- (5.5,-1);
+		
+		\draw[black, very thick] (0,0) rectangle node{$a q_3$} (6.6,0.5);
+		\draw[black, very thick] (6.6,0) rectangle node{$b q_3$} (8.8,0.5);
+		\draw[black, very thick] (8.8,0) rectangle node{$b q_2$} (11,0.5);
+		\node[] at (-0.5,0.25) {$\overline{\kappa}_{q_3}$};
+		
+		\draw[black, very thick] (0,0.75) rectangle node{$a q_2$} (4.4,1.25);
+		\draw[black, very thick] (4.4,0.75) rectangle node{$b q_1$} (7.7,1.25);
+		\draw[black, very thick] (7.7,0.75) rectangle node{$b q_3$} (11,1.25);
+		\node[] at (-0.5,1) {$\overline{\kappa}_{q_2}$};
+		
+		\draw[black, very thick] (0,1.5) rectangle node{$a q_1$} (2.2,2);
+		\draw[black, very thick] (2.2,1.5) rectangle node{$b q_1$} (6.6,2);
+		\draw[black, very thick] (6.6,1.5) rectangle node{$b q_2$} (11,2);
+		\node[] at (-0.5,1.75) {$\overline{\kappa}_{q_1}$};
+		
+		\draw (-0.2,-1.75) -- (-0.2,2);
+		\end{tikzpicture}
+		
+	\end{center}
+	
+	One can compute in polynomial time the endpoints of all intervals $[\alpha, \beta) \in \Delta$. For any $a \in \Delta$ and $r \in Q$ the image $\overline{\kappa}_r(a)$ contains exactly one element. Therefore, for each $r \in Q$ we may define a function $\kappa_r: \Delta \rightarrow \Sigma Q$ such that $\kappa_r([\alpha, \beta)) = \overline{\kappa}_r(x)$ for all $x \in [\alpha, \beta)$. We define the probability distribution $\rho$ on $\Delta$ by $\rho_{[\alpha,\beta)} = \beta - \alpha$ for all $[\alpha,\beta) \in \Delta$. The distribution $\rho$ is computable in polynomial time.
+	
+	In our example above $\Delta = \{[0,0.2), [0.2,0.4), [0.4,0.6), [0.6,0.7), [0.7,0.8), [0.8,1)\}$ and $\kappa_{q_1}$ is defined piecewise by
+	\begin{equation}
+	\kappa_{q_1}(x) = \begin{cases}
+	a q_1 & x = [0,0.2) \\
+	b q_1 & x \in \{[0.2,0.4), [0.4,0.6)\} \\
+	b q_2 & x \in \{[0.6,0.7), [0.7,0.8), [0.8, 1)\}. \\
+	\end{cases} 
+	\end{equation}
+	
+	
+	Let $r_0 \in Q$. We may extend the mapping $\kappa_{r_0}$ to a word $c~\overline{w} \in \Delta^+$ inductively by letting $\kappa_{r_0}(c~\overline{w}) = (a_1 r_1) \kappa_{r_1}(\overline{w})$ where $(a_1 r_1) = \kappa_{r_0}(c)$. We now prove (\ref{markov2indepmeasures}) by induction on the length of the word. Let $a_1 r_1 \in \Sigma Q$ then by the definition of $\kappa_{r_0}$,
+	\begin{equation*}
+	\PP_{e_{r_0}}(a_1 r_1 (\Sigma Q)^\omega) = \Psi(a_1)_{r_0, r_1} = \rho\Big(\kappa_{r_0}^{-1}(\{a_1 r_1\})\Big) = \PP_{\rho}(\kappa_{r_0}^{-1}(\{a_1 r_1\}) \Delta^\omega).
+	\end{equation*}
+	Now assume \Cref{markov2indepmeasures} holds for all words of length $n - 1 \in \NN$. Then for a word $a_1 r_1 w \in (\Sigma Q)^n$
+	\begin{align*}
+	\PP_{e_{r_0}}(a_1 r_1 w (\Sigma Q)^\omega) & = \Psi(a_1)_{r_0, r_1} \PP_{e_{r_1}}(w (\Sigma Q)^\omega) \\
+	& = \PP_{\rho}\Big(\kappa_{r_0}^{-1}(\{a_1 r_1\}) \Delta^\omega\Big) \PP_{\rho}\Big(\kappa_{r_1}^{-1}(\{w\}) \Delta^\omega\Big) \\
+	& = \PP_{\rho}\Big(\kappa_{r_0}^{-1}(\{a_1 r_1\})\kappa_{r_1}^{-1}(\{w\})\Delta^\omega\Big) \\
+	& = \PP_{\rho}\Big(\kappa_{r_0}^{-1}(\{a_1 r_1 w\}) \Delta^\omega\Big)
+	\end{align*}
+	by the independence of $\PP_{\rho}$ which completes the induction.
+\end{proof}
+
+For $\pi_1 \in [0,\infty)^{Q_1}$ and $\pi_2 \in [0,1]^{Q_2}$ we write $\pi_1 \times \pi_2 \in [0,\infty]^{Q_1 \times Q_2}$ for the vector $(\pi_1 \times \pi_2)_{(i,j)} := (\pi_1)_i  (\pi_2)_j$.
+
+\begin{proof}[Proof of \Cref{from-gen-to-nongen}]
+	By \Cref{makereduciblelyapsys}, since $(Q_2, \Sigma, \Psi_2)$ is an HMM, we may compute in polynomial time a finite set $\Delta$, a distribution $\rho \in [0,1]^{\Delta}$ and for each $r \in Q_2$ a mapping $\kappa_r : \Delta \rightarrow \Sigma Q_2$ with the property stated in \Cref{makereduciblelyapsys}. Then, we define $\tilde{\Psi}: \Delta \rightarrow [0,1]^{Q_1 \times Q_2}$ such that for all $(q_0, r_0), (q, r) \in Q_1 \times Q_2$:
+	\begin{equation*}
+	\tilde{\Psi}(\overline{a})_{(q_0, r_0), (q, r)} = \begin{cases}
+	\Psi_1(a)_{q_0, q} & \text{when }\kappa_{r_0}(\overline{a}) = a r \\
+	0 & \text{otherwise.}
+	\end{cases}
+	\end{equation*}
+	We extend $\tilde{\Psi}$ to the mapping $\tilde{\Psi} : \Delta^* \rightarrow [0,1]^{(Q_1 \times Q_2) \times (Q_1 \times Q_2)}$ by $\tilde{\Psi}(\overline{a}_1 \cdots \overline{a}_n) = \tilde{\Psi}(\overline{a}_1) \cdots \tilde{\Psi}(\overline{a}_n)$. 
+	
+	Let $r_0 \in Q_2$, $\overline{a}_1 \cdots \overline{a}_n \in \Delta^*$ and $\kappa_{r_0}(\overline{a}_1 \cdots \overline{a}_n) = a_1 r_1 \cdots a_n r_n$. By the definition of the extension of $\kappa_{r_0}$, it follows that $\land_{i = 1}^n\kappa_{r_{i - 1}}(\overline{a}_i) = a_i r_i$. For all $q_0, \dots q_n \in Q_1$ we have
+	\begin{align*}
+	\Psi_1(a_1)_{q_0, q_1} \cdots \Psi_1(a_n)_{q_{n-1}, q_n} & = \tilde{\Psi}(\overline{a}_1)_{(q_0, r_0), (q_1, r_1)} \cdots\tilde{\Psi}(\overline{a}_n)_{(q_{n-1}, r_{n-1}), (q_n, r_n)} \\
+	& = \sum_{\tilde{r}_1, \dots, \tilde{r}_n \in Q_2}\tilde{\Psi}(\overline{a}_1)_{(q_0, \tilde{r}_0), (q_1, \tilde{r}_1)} \cdots \tilde{\Psi}(\overline{a}_n)_{(q_{n-1}, \tilde{r}_{n-1}), (q_n, \tilde{r}_n)} \\
+	\end{align*}
+	and therefore by the definition of $\tilde{\Psi}$,
+	\begin{equation}\label{equalityoftildeandpsi}
+	\begin{aligned}
+	& \|(\pi_1 \times e_{r_0}) \tilde{\Psi}(\overline{a}_1 \cdots \overline{a}_n)\| \\
+	& = \sum_{q_0 \in \supp\,\pi_1}\sum_{(q_1, \tilde{r}_1), \dots (q_n, \tilde{r}_n) \in C} (\pi_1)_{q_0} \tilde{\Psi}(\overline{a}_1)_{(q_0, \tilde{r}_0), (q_1, \tilde{r}_1)} \cdots \tilde{\Psi}(\overline{a}_n)_{(q_{n-1}, \tilde{r}_{n-1}), (q_n, \tilde{r}_n)} \\
+	& = \sum_{q_0 \in \supp\,\pi_1}\sum_{q_1, \dots q_n \in Q_1} \sum_{\tilde{r}_1, \dots \tilde{r}_n \in Q_2} (\pi_1)_{q_0} \tilde{\Psi}(\overline{a}_1)_{(q_0, \tilde{r}_0), (q_1, \tilde{r}_1)} \cdots \tilde{\Psi}(\overline{a}_n)_{(q_{n-1}, \tilde{r}_{n-1}), (q_n, \tilde{r}_n)} \\
+	& = \sum_{q_0 \in \supp\,\pi_1}\sum_{q_1, \dots q_n \in Q_1} (\pi_1)_{q_0} \tilde{\Psi}(\overline{a}_1)_{(q_0, r_0), (q_1, r_1)} \cdots \tilde{\Psi}(\overline{a}_n)_{(q_{n-1}, r_{n-1}), (q_n, r_n)} \\
+	& = \sum_{q_0 \in \supp\,\pi_1}\sum_{q_1, \dots q_n \in Q_1} (\pi_1)_{q_0} \Psi_1(a_1)_{q_0, q_1} \cdots \Psi_1(a_n)_{q_{n-1}, q_n} \\
+	& = \|\pi_1 \Psi_1(a_1 \cdots a_n)\|.
+	\end{aligned}
+	\end{equation}
+	Suppose there is an edge in $G_{(Q_1, \Sigma, \Psi_1), (Q_2, \Sigma, \Psi_2)}$ between two states $(q_0, r_0), (q, r) \in C$ then there is $a \in \Sigma$ such that $\Psi_1(a)_{q_0, q} > 0$ and $\Psi_2(a)_{r_0, r} > 0$. Hence, $\PP_{e_{r_0}}(a (\Sigma Q)^\omega) > 0$ and so by \Cref{makereduciblelyapsys} there exists $\overline{a} \in \kappa_{r_0}^{-1}(\{a r\})$. It follows that $\tilde{\Psi}(\overline{a})_{(q_0, r_0), (q, r)} > 0$. Therefore, since $C$ is a bottom SCC of $G_{(Q_1, \Sigma, \Psi_1), (Q_2, \Sigma, \Psi_2)}$, we have that the graph of the matrix system $(C, \Delta, \tilde{\Psi}_{|C})$ is strongly connected and therefore $((C, \Delta, \tilde{\Psi}_{|C}), \rho)$ is a Lyapunov system. Moreover, for any $\pi_1 \in [0,1]^{Q_1}$ and $\pi_2 \in [0,1]^{Q_2}$ such that $\supp(\pi_1) \times \supp(\pi_2) \subseteq C$ we have that $\| (\pi_1 \times \pi_2) \tilde{\Psi}(\overline{a}_1 \cdots \overline{a}_n) \| = \| (\pi_1 \times \pi_2)_{|C} \tilde{\Psi}_{|C}(\overline{a}_1 \cdots \overline{a}_n) \|$ where $(\pi_1 \times \pi_2)_{|C}$ is the truncation of the vector $\pi_1 \times \pi_2$ to $C$. Further,  we have for all $x \in \RR$ and $n \in \NN$
+	\begin{equation}\label{equalityofdistributionspitorho}
+	\begin{aligned}
+	& \PP_{\pi_2}( \{ w \in \Sigma^\omega \mid \| \pi_1 \Psi(w_n) \| = x \}). \\
+	& = \sum_{r_0 \in \supp\,\pi_2} (\pi_2)_{r_0} \PP_{e_{r_0}}( \{ w \in \Sigma^\omega \mid \| \pi_1 \Psi_1(w_n) \| = x \}) \\
+	& = \sum_{r_0 \in \supp\,\pi_2} (\pi_2)_{r_0} \sum_{a_1 r_1 \cdots a_n r_n \in (\Sigma Q_2)^n \text{ s.t. }\| \pi_1 \Psi_1(a_1 \cdots a_n) \| = x} \PP_{e_{r_0}}(a_1 r_1 \cdots a_n r_n(\Sigma Q)^\omega) \\
+	& = \sum_{r_0 \in \supp\,\pi_2} (\pi_2)_{r_0} \sum_{a_1 r_1 \cdots a_n r_n \in (\Sigma Q_2)^n \text{ s.t. }\| \pi_1 \Psi_1(a_1 \cdots a_n) \| = x} \PP_{\rho}(\kappa_{r_0}^{-1}(a_1 r_1 \cdots a_n r_n)(\Delta)^\omega) \\
+	& \quad \text{by \Cref{makereduciblelyapsys}} \\
+	& = \sum_{r_0 \in \supp\,\pi_2} (\pi_2)_{r_0} \PP_{\rho}(\{\overline{w} \in \Delta^\omega \mid \kappa_{r_0}(\overline{w}_n) = a_1 r_1 \cdots a_n r_n,~ \| \pi_1 \Psi_1(a_1 \cdots a_n) \| = x\}) \\
+	& = \sum_{r_0 \in \supp\,\pi_2} (\pi_2)_{r_0} \PP_{\rho}( \{ \overline{w} \in \Delta^\omega \mid \| (\pi_1 \times e_{r_0}) \tilde{\Psi}(\overline{w}_n) \| = x \}) \quad \text{by (\ref{equalityoftildeandpsi})} \\
+	& = \sum_{r_0 \in \supp\,\pi_2} (\pi_2)_{r_0} \PP_{\rho}( \{ \overline{w} \in \Delta^\omega \mid \| (\pi_1 \times e_{r_0})_{|C} \tilde{\Psi}_{|C}(\overline{w}_n) \| = x \}).
+	\end{aligned}
+	\end{equation}
+	Combining the above equalities with \Cref{lem:lyapunov-exponent} we have that there exists a $\lambda \in [-\infty, 0]$ which does not depend on $\pi_1$ or $\pi_2$ such that 
+	\begin{align*}
+	1 & = \sum_{r_0 \in \supp \, \pi_2} (\pi_2)_{r_0} \\
+	& = \sum_{{r_0} \in \supp \, \pi_2} (\pi_2)_{r_0} \PP_{\rho}\Big( \Big\{ \overline{w} \in \Delta^\omega \mid \lim_{n \rightarrow \infty} \frac1n \ln \| (\pi_1 \times e_{r_0})_{|C} \tilde{\Psi}_{|C}(\overline{w}_n) \| \in \{-\infty, \lambda\} \Big\}\Big) \text{ by \Cref{lem:lyapunov-exponent}} \\
+	& = \PP_{\pi_2}\Big( \Big\{w \in \Sigma^\omega \mid \lim_{n \rightarrow \infty} \frac1n \ln \| \pi_1 \Psi(w_n) \| \in \{-\infty, \lambda\} \Big\}\Big) \text{ by (\ref{equalityofdistributionspitorho})}.
+	\end{align*}
+\end{proof}
+
+
+\subsection{Proof of \Cref{lem:construct-L-systems}}
+
+Towards a proof of \Cref{lem:construct-L-systems} we make some additional definitions. A \emph{reducible Lyapunov system} is a Lyapupov system $((Q, \Sigma, \Psi),\rho)$ except that the graph $G = (Q, E)$ with $E = \{(q, r) \mid \sum_{a \in \Sigma} \Psi_{q, r}(a) > 0\}$ is not necessarily strongly connected. For sets $U, V \subseteq Q$ we write $U \rightarrow_{G} V$ if there is $u \in U$ and $v \in V$ such that $v$ is reachable from $u$ in $G$.
+
+We use the following technical lemmas. 
+
+\begin{theorem}[F{\"u}rstenberg–Kesten theorem]\label{furstenbergkesten}
+Let $((Q, \Sigma, \Psi), \mu)$ be a reducible Lyapunov system then there exists $\lambda \in [-\infty, \infty)$ such that $\PP_{\rho}$-a.s. we have
+\begin{equation}
+\lim_{n \rightarrow \infty} \frac1n \ln \|\vec{1} \Psi(w_n)\| = \lambda.
+\end{equation}
+\end{theorem}
+
+The following lemma is Theorem 1.1 from \cite{germicorl08}.
+
+\begin{lemma}\label{fullsupportlyapdecomp}
+Let $\Sigma$ be a finite set of observations, $\rho \in [0,1]^\Sigma$ and let $((Q_1, \Sigma, \Psi_1), \rho), ((Q_2, \Sigma, \Psi_2), \rho)$ be reducible Lyapunov systems. By \Cref{furstenbergkesten} there exists $\lambda_1, \lambda_2 \in [-\infty, \infty)$ such that for $i = 1, 2$ we have
 \begin{equation*}
-\Phi(a')_{(q_1,q_2),(r_1,r_2)} = \begin{cases}
-\Psi(a)_{q_1, r_1} & (r_2, a) \in \kappa_{q_2}^{-1}(a') \\
-0 & \text{else}. \\
-\end{cases}
-\end{equation*} 
-The triple $\mathcal{M} = (Q', \Sigma', \Phi)$ is a matrix system with a strongly connected graph due to $C$ being a bottom SCC. The pair $\mathcal{S'} = (\mathcal{M}, \MLeb)$ is a Lyapunov system (a representation of) which can be computed in $O(|Q_2|^2|Q_1|^2 |\Sigma|)$ time. 
+\lim_{n\rightarrow \infty} \frac1n \ln \|\vec{1} \Psi_i(w_n) \| = \lambda_i.
+\end{equation*}
+Further, let $\Psi_{12} : \Sigma \rightarrow [0,1]^{Q_1 \times Q_2}$ specify transition from $Q_1$ to $Q_2$ and define $\Psi^* : \Sigma \rightarrow [0,1]^{(Q_1 \cup Q_2) \times (Q_1 \cup Q_2)}$ block-wise as 
+\begin{equation*}
+\Psi^*(a) = \begin{pmatrix}
+\Psi_1(a) & \Psi_{12}(a) \\
+0 & \Psi_2(a)
+\end{pmatrix}.
+\end{equation*}
+It follows $((Q_1 \cup Q_2, \Sigma, \dot{\Psi}), \rho)$ is a reducible Lyapunov system and
+\begin{equation*}
+\lim_{n\rightarrow \infty} \frac1n \ln \|\vec{1} \dot{\Psi}(w_n) \| = \max \{\lambda_1, \lambda_2\}.
+\end{equation*}
+\end{lemma}
 
-Given a starting state $r_0$ we may extend the mapping $\kappa_{r_0} : [0,1)^n \rightarrow (Q_2 \times \Sigma)^n$ for $n \in \NN$ by letting $\kappa_{r_0}(a'w) = (a, r_1) \kappa_{r_1}(w)$ where $\kappa_{r_0}(a') = (a, r_1)$. Fix $(r_1, a_1) \cdots (r_n, a_n) \in (Q_2 \times \Sigma)^n$ and let $C^k = \{q_1 \cdots q_n \in Q_1^n \mid (q_1, r_1), \dots, (q_k, r_k) \in C\}$ for $k \leq n$. For a word $w' = a_1' \cdots a_n' \in \{\kappa_{j_0}(a_1' \dots a_n') = (r_1, a_1), \cdots, (r_n, a_n)\}$ and start and end states $(q_0, r_0)$ and $(q_n, r_n)$ respectively, we have
-\begin{align*}
-\Phi(w')_{(q_0, r_0), (q_n, r_n)} & = \sum_{(q_1, \dots, q_{n-1}) \in C^1} \Phi(a_1')_{(q_0, r_0),(q_1,r_1)} \dots \Phi(a_n')_{(q_{n - 1}, r_{n - 1}),(q_n,r_n)}\\
-& = \sum_{(q_1, \dots, q_{n-1}) \in C^{n-1}} \Psi(a_1)_{q_0, q_1} \dots \Psi(a_n)_{q_{n - 1}, q_n}\\
-& = \Psi(a_1 \cdots a_n)_{q_0, q_n}.
-\end{align*}
-Further, we have
-\begin{align*}
-\Psi(a_1)_{r_0, r_1} \dots \Psi(a_n)_{r_{n - 1}, r_n} & = \sum_{a_1' \cdots a_n' \in [0,1)^n} \MLeb(a_1' \times \dots \times a_n')\1_{\kappa_{r_0}(a_1' \dots a_n') = (r_1, a_1), \cdots, (r_n, a_n)}\\
-& = \PP_{\MLeb}(\kappa_{r_0}(a_1' \dots a_n') = a_1 \dots a_n).
-\end{align*}
-Write $\pi_1 \times \pi_2$ for the distribution on $C$ given by $(\pi_1 \times \pi_2)_{q,r} = (\pi_1)_q (\pi_2)_r$. It follows from the above that for any measurable set $A \subseteq \RR$, we have
+By generalising \Cref{fullsupportlyapdecomp}
+
+\begin{lemma}\label{reduclyapsys}
+Let $((Q, \Sigma, \Psi), \rho)$ be a reducible Lyapunov system and suppose $(Q, E)$ has strongly connected components $C_1, \dots, C_K$. Let $\,\mathbf{0}$ be the zero matrix and let
 \begin{equation*}
-\PP_{\pi_2}(\pi_1 \Psi(a_1\cdots a_n) \in A) = \PP_{\MLeb}(\pi_1 \times \pi_2 \Phi(a_1'\cdots a_n') \in A)
+\mathcal{Z} = \{C \in \{C_1, \dots , C_K\} \mid \exists u \in \Sigma^* \text{ s.t. }\Psi_{|C}(u) = \mathbf{0} \}.
 \end{equation*}
-which implies both points in the lemma.
-\end{proof}
+For each $k \in [K]$, $\mathcal{G}_k := ((C_k, \Sigma, \Psi_{|C_k}), \rho)$ is a Lyapunov system. We have that $\PP_{\rho}$-almost surely,
+\begin{equation} \label{furstenberggroups}
+\lim_{n\rightarrow \infty} \frac1n \ln \|\vec{1} \Psi(w_n) \| = \max \Big( \Big\{\lambda(\mathcal{G}_k) \mid C_k \notin \mathcal{Z} \Big\} \cup \{-\infty\} \Big) 
+\end{equation}
+where $\vec{1}$ is the row vector all of whose entries are $1$. Further, for any initial distribution $\pi \in [0,1]^Q$, we have that $\PP_{\rho}$-almost surely,
+\begin{equation}\label{generalizedfursten}
+\lim_{n\rightarrow \infty} \frac1n \ln \|\pi \Psi(w_n) \| \in \Big\{\lambda(\mathcal{G}_k) \mid \supp~\pi  \rightarrow_{G} C_k, C_k \notin \mathcal{Z} \Big\} \cup \{-\infty\}.
+\end{equation}
+\end{lemma}
 
-\constructLsystems*
+\begin{proof}
+We first prove (\ref{furstenberggroups}). By \Cref{furstenbergkesten} for $i \in [N]$ there exists $\lambda_i \in [-\infty, \infty)$ such that $\PP_{\rho}$-a.s.,
+\begin{equation*}
+\lim_{n\rightarrow \infty} \frac1n \ln \|\vec{1} \Psi_{|C_i}(w_n) \| = \lambda_i.
+\end{equation*}
+In the case $\lambda_i = -\infty$ then by \Cref{lem:lyapunov-exponent} we have that $\PP_{\rho}$-a.s. there is a word $u \in \Sigma^*$ such that $\vec{1} \Psi_{|C_i}(u) = \vec{0}$ hence $C_i \in \mathcal{Z}$. 
 
-\begin{proof}
-We define the following sets
+In the case $\lambda_i \in \RR$ then by \Cref{lem:lyapunov-exponent} $\lambda_i = \lambda(\mathcal{G}_i)$. Also $\{w \in \Sigma^\omega \mid \exists n\in\NN : \vec{1}\Psi_{|C_i}(w_n) = \vec{0}\}$ is $\PP_{\rho}$-null set and therefore empty because $\rho$ has full support and therefore all finite words have positive probability of being produced. It follows that $C_i \notin \mathcal{Z}$.
+
+We proceed by induction. In the case $K = 1$, the cases described previously immediately imply that (\ref{furstenberggroups}) holds. Now we assume the lemma holds for some $K = m \in \NN$. We prove this implies the theorem holds for $K = m + 1$.
+
+Let $((Q, \Sigma, \Psi), \rho)$ be a reducible Lyapunov system such that $(Q, E)$ has strongly connected components $C_1, \dots, C_{m + 1}$. We have that $((C_1 \cup \cdots \cup C_m, \Sigma, \Psi_{|C_1 \cup \cdots \cup C_m}), \rho)$ is a reducible Lyapunov system so by the induction hypothesis, $\PP_{\rho}$-a.s. we have
+\begin{equation*}
+\lim_{n\rightarrow \infty} \frac1n \ln \|\vec{1} \Psi_{|C_1 \cup \cdots \cup C_m}(w_n) \| = \max\Big(\{\lambda(\mathcal{G}_i) \mid i \in [m], C_i \notin \mathcal{Z}\} \cup \{-\infty\}\Big).
+\end{equation*}
+In the case that $\lambda_{m + 1} \in \RR$ then $\lambda(\mathcal{G}_{m+1}) = \lambda_{m+1}$ and $C_{m + 1} \notin \mathcal{Z}$. Therefore, $\lambda_{m + 1} \in \{\lambda(\mathcal{G}_i) \mid i \in [m + 1], C_i \notin \mathcal{Z}\}$.
+
+In the case $\lambda_{m + 1} = -\infty$, then $C_{m + 1} \in \mathcal{Z}$ and clearly $\{\lambda(\mathcal{G}_i) \mid i \in [m], C_i \notin \mathcal{Z}\} = \{\lambda(\mathcal{G}_i) \mid i \in [m + 1], C_i \notin \mathcal{Z}\}$. So by \Cref{fullsupportlyapdecomp} we have
 \begin{align*}
-C^* & = \{(q,r) \in Q \times Q \mid \supp (\pi_1) \times \supp (\pi_2) \rightarrow_{G_{\mathcal{H}, \mathcal{H}}} \{(q, r)\}, (q, r) \in R \text{ for some } R \in \mathcal{R}\} \\
-C_0 & = C^* \cap \{(q,r) \in Q \times Q \mid (q,r) \text{ is in a bottom SCC of }G_{\mathcal{H}, \mathcal{H}} \} \\
+\lim_{n\rightarrow \infty} \frac1n \ln \|\vec{1} \Psi(w_n) \| & = \max\Big\{\lambda_{m + 1}, \max\Big(\{\lambda(\mathcal{G}_i) \mid i \in [m], C_i \notin \mathcal{Z}\} \cup \{-\infty\} \Big) \Big\} \\
+& = \max \Big(\{\lambda(\mathcal{G}_i) \mid i \in [m + 1], C_i \notin \mathcal{Z}\} \cup \{-\infty\} \Big).
 \end{align*}
-Conditioned on a produced word $r_0 a_1 r_1 \cdots a_m r_m \in (\supp~\pi_2)(\Sigma Q)^*$ we have
-\begin{align*}
-\lim_{n \rightarrow \infty}\frac1n \ln\frac{\|\pi_1 \Psi(a_1 \cdots a_m) \Psi(w_n)\|}{\|\pi_2 \Psi(a_1 \cdots a_m) \Psi(w_n)\|} & = \lim_{n \rightarrow \infty}\frac1n \ln\frac{\|\pi_1 \Psi(a_1 \cdots a_m) \Psi(w_n)\|}{\|\delta_{r_m} \Psi(w_n)\|} \\
-& - \lim_{n \rightarrow \infty}\frac1n \ln\frac{\|\pi_2 \Psi(a_1 \cdots a_m) \Psi(w_n)\|}{\|\delta_{r_m} \Psi(w_n)\|} \\
-& = \max_{q \in \supp~ \pi_1 \Psi(a_1 \cdots a_m)}\lim_{n \rightarrow \infty}\frac1n \ln\frac{\|\delta_q \Psi(w_n)\|}{\|\delta_{r_m} \Psi(w_n)\|}.
-\end{align*}
-The state $r_m$ is $\PP_{\pi_2}$-almost surely in a bottom SCC of $\sum_{a \in \Sigma} \Psi(a)$. Hence, we have $\Lambda_{\pi_1,\pi_2} \subset \{\ell \in \bigcup_{R \in \mathcal{R}}\Lambda_{\delta_q, \delta_r} \mid (q, r) \in C^*\}$ since . We then define subsets $C_0 \subseteq C_1 \subseteq \cdots \subseteq C_M = C^*$ and then prove the claim
-\begin{equation}\label{indclaimsccs}
-\{\ell \in \Lambda_{\delta_q, \delta_r} \mid (q, r) \in C_m\} \subseteq \{-\infty\} \cup \{\lambda(\mathcal{S}^1_R) - \lambda(\mathcal{S}^2_R) \mid R \in \mathcal{R}, R \subseteq C^*\}
-\end{equation}
-for all $m \leq M$ by induction. 
-
-Consider the case $(q, r) \in C_\text{b}$ then for a word $r a_1 r_1 \cdots a_m r_m \in r(\Sigma Q)^*$ since $r_m$ is in a bottom SCC of $\sum_{a \in \Sigma}\Psi(a)$ we have that $(q, r)$ and $(r, r)$ are both in bottom SCCs of $G_{\mathcal{H}, \mathcal{H}}$. Hence, there are right-bottom SCCs $R$ and $R'$ such that 
+We now prove (\ref{generalizedfursten}). Like in \Cref{sec:qual}, for $S \subseteq Q$ and $a\in\Sigma$, define $\delta'(S, a) = \{q' \in Q \mid \exists\, q \in S : \Psi(a)_{q, q'} > 0\}$. Then we define the Markov chain $\mathcal{B}' := (2^Q, T')$ where
 \begin{equation*}
-\lim_{n\rightarrow \infty} \frac1n \ln \frac{\|\delta_q \Psi(a_1 \cdots a_m)\|}{\|\delta_r \Psi(a_1 \cdots a_m)\|} = \lim_{n\rightarrow \infty} \frac1n \ln \frac{ \| \delta_{(q, r)} \overline{\Psi}_{|R}(a_1 r_1 \cdots a_m r_m) \|}{\| \delta_{(r, r)} \overline{\Psi}_{|R'}(a_1 r_1 \cdots a_m r_m) \|} \in \{-\infty, \lambda(S^1_R) - \lambda(S^2_R)\}.
+T'_{S, S'} := \sum_{\delta'(S, a) = S'} \rho(a).
 \end{equation*}
+Let $\mathcal{D}$ be the set of bottom SCCs that are reachable in $\mathcal{B}'$ from the initial state $\supp~\pi$. We fix $D \in \mathcal{D}$. We may order the $C_1 \cdots C_K$ such that for some $k \in [K]$
+\begin{equation*}
+S_D := \{q \in S \mid S \in D \} \cap C_i \neq \emptyset
+\end{equation*}
+for all $i \in [k]$. It is clear that $S_D \subseteq C_1\cup \cdots \cup C_k$. We show the reverse inclusion. Let $i \in [k]$ then there is $q_0 \in C_i \cap S_D$. For any $q' \in C_i$ there is a word $a_1 q_1 \cdots a_m q_m \in (\Sigma Q)^*$ such that $q_m = q'$ and $\Psi_{q_{i - 1}, q_i}(a_i) > 0$ for all $i \in [m]$. It follows that $q' \in S_D$ and therefore $S_D = C_1 \cup \cdots \cup C_k$.
 
-Write $R_1, \dots, R_M \subseteq C^*$ for the remaining right-bottom SCCs in $C^*$ ordered in such a way that $R_i \rightarrow_{G_{\mathcal{H}, \mathcal{H}}} R_j$ implies $i \geq j$. This ordering exists due to the DAG structure of right-bottom SCCs under the $\rightarrow_{G_{\mathcal{H}, \mathcal{H}}}$ transitive relation. We define $C_{m+1} = C_m \cup R_{m+1}$. Assume the claim given in \Cref{indclaimsccs} holds for some $C := C_m$. All outgoing transitions of $R := R_{m+1}$ go to states in $C$. Consider the block matrix system $(C \cup R, \Sigma \times Q_R, \overline{\Psi}_{|C \cup R})$. Then for $a \in \Sigma$, we have the block definition 
+We have that $\PP_{\rho}$-a.s. $\lim_{n \rightarrow \infty} \frac1n \ln \|\vec{1} \Psi_{|S_D}(w_n)\|$ exists and equals 
 \begin{equation*}
-\overline{\Psi}_{|C \cup R}(a) = \begin{pmatrix}
-\overline{\Psi}_{|R}(a) && T\\
-0 && \overline{\Psi}_{|C}(a) \\
-\end{pmatrix}
+\lambda_D := \max\Big(\{\lambda(\mathcal{G}_i) \mid i \in [k], C_i \notin \mathcal{Z}\} \cup \{-\infty\}\Big)
 \end{equation*}
-where $T$ is a matrix representing the transitions from the sets of states $R$ to $C$. Let $w \in (\Sigma Q_R)^\omega$ with prefix $w_n = a_1 r_1 \cdots a_n r_n \in (\Sigma Q_R)^n$ (we assume $n \geq 3$). We write $w_{k+1, n}$ for the word $a_{k+1} r_{k+1} \cdots a_n r_n$. It follows that
+by (\ref{furstenberggroups}). In particular there is $q \in S_D$ such that
 \begin{equation*}
-\overline{\Psi}_{|C \cup R}(w_n) = \begin{pmatrix}
-\overline{\Psi}_{|R}(w_n) && \sum_{k = 1}^{n}\overline{\Psi}_{|R}(w_{k-1}) T(a_k r_k) \overline{\Psi}_{|C}(w_{k+1, n})\\
-0 && \overline{\Psi}_{|C}(w_n) \\
-\end{pmatrix}
-\end{equation*}
-where $w_0$ and $w_{n+1, n}$ are both interpreted as the empty word $\epsilon$. If $(q, r) \in C$ then \Cref{indclaimsccs} holds immediately so assume $(q,r) \in R$. Therefore if the limits exist, 
+\alpha := \PP_{\rho}\Big(\lim_{n \rightarrow \infty} \frac1n \ln \|e_q \Psi(w_n)\| = \lambda_D\Big) = \PP_{\rho}\Big(\lim_{n \rightarrow \infty} \frac1n \ln \|e_q \Psi_{|S_D}(w_n)\| = \lambda_D\Big) > 0.
+\end{equation*} 
+For all $S_0 \in D$ there is a sequence $a_1 S_1 \cdots a_n S_n \in (\Sigma D)^*$ such that $q \in S_n$ and $S_{i} = \delta(S_{i - 1}, a_i)$ for all $i = 1, \dots, n$. We have that $\beta_{S_0} := \prod_{i = 1}^n \rho(a_i) > 0$. Write $\beta = \min \{\beta_{S_0} \mid S_0 \in D\}$. 
+Let $\pi' \in [0,1]^Q$ be such that $\supp~\pi' \in D$. Then for any $u \in \Sigma^*$ we have 
 \begin{align*}
-\lim_{n \rightarrow \infty} \frac1n \ln \|e_{(q,r)} \overline{\Psi}_{|C \cup R}(w_n) \| & = \lim_{n \rightarrow \infty} \frac1n \ln \|e'_{(q,r)} \big[~ \overline{\Psi}_{|R}(w_n) \\
-& + \sum_{k = 1}^{n}\overline{\Psi}_{|R}(w_{k-1}) T(a_k r_k) \overline{\Psi}_{|C}(w_{k+1, n})\big]\| \\
-& = \lim_{n \rightarrow \infty} \frac1n \ln \|e'_{(q,r)} \sum_{k = 1}^{n}\overline{\Psi}_{|R}(w_{k-1}) T(a_k r_k) \overline{\Psi}_{|C}(w_{k+1, n})\| \\
-& = \lim_{n \rightarrow \infty} \max_{k \leq n}\frac1n \ln \|e'_{(q,r)} \overline{\Psi}_{|R}(w_{k-1}) T(a_k r_k) \overline{\Psi}_{|C}(w_{k+1, n})\| \\
-& \geq \max \Big\{ \lim_{n \rightarrow \infty} \frac1n \ln \| e'_{q, r}\overline{\Psi}_{|R}(w_n) \|,\\
-& \sup_{k \in \NN} \lim_{n \rightarrow \infty}\frac1n \ln \|e'_{(q,r)} \overline{\Psi}_{|R}(w_{k-1}) T(a_k r_k) \overline{\Psi}_{|C}(w_{k+1, n})\| \Big\} \\
+& \PP_{\rho}(\lim_{n \rightarrow \infty} \frac1n \ln \|\pi' \Psi(w_n)\| = \lambda_D \mid u \Sigma^\omega) \\
+& = \PP_{\rho}(\lim_{n \rightarrow \infty} \frac1n \ln \|\pi' \Psi(w_n)\| = \lambda_D \mid u \Sigma^\omega) \\
+& \geq \beta \PP_{\rho}(\lim_{n \rightarrow \infty} \frac1n \ln \|\pi' \Psi(u w_n)\| = \lambda_D) \\
+& \geq \beta \PP_{\rho}(\lim_{n \rightarrow \infty} \frac1n \ln \|e_q \Psi(w_n)\| = \lambda_D) \\
+& = \beta \alpha > 0.
 \end{align*}
-where $e'_{(q,r)}$ is the dirac distribution for the state $(q,r) \in R$. Write $((i_1, j_1),(i_2, j_2))_k \in \supp T(a_k)$ for a possible transition from $R$ to $C$. Further, for such a transition write 
+Hence by L{\'e}vy's 0-1 law we have 
 \begin{align*}
-X_R & :=  \lim_{k \rightarrow \infty} \frac{1}{k} \ln \| e'_{(q, r)}\overline{\Psi}_{|R}(w_{k-1}) T(a_k r_k) \| \\
-& = \lim_{M \rightarrow \infty} \sup_{k \geq M} \frac{1}{k} \ln \| e'_{(q, r)}\overline{\Psi}_{|R}(w_{k-1}) T(a_k r_k) \|\\
-X_C^k & := \lim_{n \rightarrow \infty}\frac1n \ln \|e'_{(q,r)} \overline{\Psi}_{|R}(w_{k-1}) T(a_k r_k) \overline{\Psi}_{|C}(w_{k+1, n})\| \\
-&= \lim_{M \rightarrow \infty} \sup_{n \geq M} \frac1n \ln \|e'_{(q,r)} \overline{\Psi}_{|R}(w_{k-1}) T(a_k r_k) \overline{\Psi}_{|C}(w_{k+1, n})\|.
+1 & = \PP_{\rho}\Big(\lim_{n \rightarrow \infty} \frac1n \ln \|\pi' \Psi(w_n)\| = \lambda_D\Big) \\
+& = \PP_{\rho}\Big(\lim_{n \rightarrow \infty} \frac1n \ln \|\pi' \Psi(w_n)\| \in \{\lambda(\mathcal{G}_i) \mid \supp~\pi \rightarrow_G C_i, C_i \notin \mathcal{Z}\} \cup \{-\infty\}\Big)
 \end{align*}
-Let $I(w_k)$ be the characteristic vector of $\supp~ e'_{(q,r)} \overline{\Psi}_{|R}(w_{k-1}) T(a_k r_k)$ then clearly $X_C^k = \lim_{n \rightarrow \infty}\frac1n \ln \|I(w_k) \overline{\Psi}_{|C}(w_{k+1, n})\|$. 
+where the last equality follows because $D \in \mathcal{D}$ is reachable from $\supp~\pi$ in $\mathcal{B}'$ which implies that for any $C_i \subseteq S_D$ we have $\supp~\pi \rightarrow_G C_i$.
 
-Since $I$ takes a finite number of values and since convergence almost surely implies convergence in probability, for all $\epsilon, \delta > 0$ there exists a $K \in \NN$ such that for all $M \geq K$
+We now relax the dependence on $D$. For any $D \in \mathcal{D}$, let $F_D = \{w \in \Sigma^\omega \mid \exists n\in\NN : \supp~(\pi \Psi(w_n)) \in D\}$. Then,
 \begin{equation*}
-\PP_{e_r}\Big( \sup_{k \geq M} |\frac{1}{k} \ln \| e'_{(q, r)}\overline{\Psi}_{|R}(w_{k-1}) T(a_k r_k) \| - X_R | \leq \epsilon \Big) \geq 1 - \delta
+\PP_{\rho}\Big( \bigcup_{D \in \mathcal{D}}F_D\Big) = 1.
 \end{equation*}
-and
-\begin{equation*}
-\PP_{e_r}\Big( |\sup_{n - k - 1\geq M} \frac{1}{n - k - 1} \ln \| I(w_k)\overline{\Psi}_{|C}(w_{k+1, n}) \| - X^k_C | \leq \epsilon \Big) \geq 1 - \delta.
-\end{equation*}
-It follows that for arbitrary $M \geq 2K+1$ 
+Write $\Theta = \{\lambda(\mathcal{G}_i) \mid \supp~\pi \rightarrow_G C_i, C_i \notin \mathcal{Z}\} \cup \{-\infty\}$ then $\PP_{\rho}$-a.s. we have
 \begin{align*}
-& \PP_{e_r}\Big( \sup_{n \geq M, K \leq k \leq n - K - 1} |\frac1n \ln \| e'_{q, r}\overline{\Psi}_{|R}(w_{k-1}) T(a_k r_k) \overline{\Psi}_{|C}(w_{k+1, n}) \| - \big[\frac{k}{n} X_R + \frac{n - k - 1}{n} X^k_C \big] | \leq \epsilon \Big) \\ 
-& = \PP_{e_r}\Big( \sup_{n \geq M, K \leq k \leq n - K - 1} \Big|\frac1n \ln \| e'_{(q, r)}\overline{\Psi}_{|R}(w_{k-1}) T(a_k r_k) \| \\
-& + \frac1n \ln \|I(w_k)\overline{\Psi}_{|C}(w_{k+1, n}) \| - \big[\frac{k}{n} X_R + \frac{n - k - 1}{n} X^k_C \big] \Big| \leq \epsilon \Big) \\
-& = \PP_{e_r}\Big( \sup_{n \geq M, K \leq k \leq n - K - 1} \frac{k}{n} \Big| \frac{1}{k} \ln \| e'_{(q, r)}\overline{\Psi}_{|R}(w_{k-1}) T(a_k r_k) \| -  X_R \Big|\\
-& + \sup_{n \geq M, K \leq k \leq n - K - 1}  \frac{n - k - 1}{n} \Big| \frac{1}{n - k - 1} \ln \|I(w_k)\overline{\Psi}_{|C}(w_{k+1, n}) \| -  X^k_C \Big| \leq \epsilon \Big) \\
-& = \PP_{e_r}\Big( \sup_{n \geq M, K \leq k \leq n - K - 1} \frac{k}{n} \Big| \frac{1}{k} \ln \| e'_{(q, r)}\overline{\Psi}_{|R}(w_{k-1}) T(a_k r_k) \| -  X_R \Big|\\
-& + \sup_{n \geq M, K \leq k \leq n - K - 1}  \frac{n - k - 1}{n} \Big| \frac{1}{n - k - 1} \ln \|I(w_k)\overline{\Psi}_{|C}(w_{k+1, n}) \| -  X^k_C \Big| \leq \epsilon \Big) \\
-& \geq \PP_{e_r}\Big( \big| \| e'_{(q, r)}\overline{\Psi}_{|R}(w_{k-1}) T(a_k r_k) \| -  X_R \big| \leq \epsilon \\
-& \land \sup_{n \geq M}\big| \frac{1}{n - k - 1} \ln \|I(w_k)\overline{\Psi}_{|C}(w_{k+1, n}) \| -  X^k_C \big| \leq \epsilon \Big)
+\PP_{\rho}(\lim_{n \rightarrow \infty} \frac1n \ln \|\pi \Psi(w_n)\| \in \Theta) & = \sum_{D \in \mathcal{D}} \PP_{\rho}(\{\lim_{n \rightarrow \infty} \frac1n \ln \|\pi \Psi(w_n)\| \in \Theta \} \mid F_D) \PP_{\rho}(F_D) \\
+& = \sum_{D \in \mathcal{D}} \PP_{\rho}(F_D) = 1.
 \end{align*}
+\end{proof}
 
 
+The following is also repeated from \Cref{sec:rep}.
 
+\definitionsforgenlyap
 
- and $n - k \geq K$
 
+\constructLsystems*
 
+\begin{proof}
+Let $\mathcal{H} = (Q, \Sigma, \Psi)$ and observe that 
+\begin{equation*}
+\PP_{\pi_2}\Big(r_0 a_1 r_1 a_2 r_2 \cdots \in Q (\Sigma Q)^\omega \mid \exists k \in \NN \text{ s.t. } r_k \text{ is in a bottom SCC of } \mathcal{H} \Big) = 1.
+\end{equation*}
+Consider a word $a_1 r_1 a_2 r_2 \cdots \in (\Sigma Q)^\omega$ such that $\PP_{\pi_2}(Q a_1 r_1 \cdots a_m r_m (\Sigma Q)^\omega) > 0$ for all $m \in \NN$ and further, there exists a $k \in \NN$ such that $r_k \in P$ where $P \subseteq Q$ is a bottom SCC of $\mathcal{H}$. We write $u = a_1 r_1 \cdots a_k r_k$ and $w = a_{k+1} r_{k+1} a_{k+2} r_{k+2}\cdots \in (\Sigma Q)^\omega$. Let $\mu_i = \pi_i \Psi(u) \times e_{r_k}$ for $i = 1,2$. Recall the definition of $\overline{\Psi}$. We have that for any $n > k$ that $\| \pi_i \Psi(a_1 \cdots a_{k + n}) \| = \| \pi_i \Psi(a_1 \cdots a_k) \Psi(a_{k+1} \cdots a_{k + n}) \| = \| \mu_i \overline{\Psi}(w_n) \|$ for $i = 1, 2$. We fix $u$ and consider words $w$ produced by $\mathcal{H}$ with initial distribution $e_{r_k}$. We have that $\PP_{e_{r_k}}$-almost surely if the limits exist,
+\begin{align*}
+\lim_{n \rightarrow \infty} \frac{1}{k + n} \ln L_{k + n}(uw) & = \lim_{n \rightarrow \infty}  \frac{1}{k + n} \Big[ \ln \| \pi_1 \Psi(a_1 \cdots a_{k + n}) \| - \ln \|\pi_2 \Psi(a_1 \cdots a_{k + n}) \| \Big] \\
+& = \lim_{n \rightarrow \infty} \frac{1}{k + n} \Big[ \ln \| \mu_1 \overline{\Psi}(w_n) \| - \ln \|\mu_2 \overline{\Psi}(w_n) \| \Big] \\
+& = \lim_{n \rightarrow \infty} \frac1n \Big[ \ln \| \mu_1 \overline{\Psi}(w_n) \| - \ln \|\mu_2 \overline{\Psi}(w_n) \| \Big] \\
+\end{align*}
+since $\lim_{n \rightarrow \infty} \frac{n}{k + n} = 1$.
 
+By \Cref{makereduciblelyapsys} there is a finite set $\Delta$, distribution $\rho \in (0,1]^{\Delta}$ and mapping $\kappa_{r_k}: \Delta^+ \rightarrow (\Sigma Q)^+$ such that $\PP_{\rho}(\{\kappa_{r_k}^{-1}(w_n \}) \Delta^\omega) = \PP_{e_{r_k}}(w_n (\Sigma Q)^\omega)$ for all $n \in \NN$. Let $S \subseteq Q \times Q$. It follows that for each $n \in \NN$ and $A \in [0, 1]^{S\times S}$ we have
+\begin{equation}\label{equalityofpushforward}
+\PP_{e_{r_k}}(\{w \in (\Sigma Q)^\omega \mid \overline{\Psi}_{|S}(w_n) = A\}) = \PP_{\rho}(\{\overline{w} \in \Delta^\omega \mid \overline{\Psi}_{|S} (\kappa_{r_k}(\overline{w}_n)) = A \}).
+\end{equation}
 
+Let $\mathcal{C}$ be the set of SCCs of $G_{\mathcal{H}, \mathcal{H}}$. We define $\sigma : \mathcal{C} \rightarrow \mathcal{P}(Q)$ such that $\sigma(R) = \{q \in Q \mid \exists p \in Q \text{ s.t. }(p,q) \in R\}$. Recall that $r_k \in P$ and $P$ is a bottom SCC. Thus, for all $i = 1, 2$, $n \in \NN$ and $(p, q) \in \supp~ ( \mu_i \overline{\Psi}(w_n))$ we have $q \in P$. Therefore, for all $R \in \mathcal{C}$ 
+\begin{equation}\label{staysinP}
+\supp~\mu_i \rightarrow_{G_{\mathcal{H}, \mathcal{H}}} R \implies \sigma(R) = P.
+\end{equation}
+Consider the composition $\overline{\Psi} \circ \kappa_{r_k} : \Delta^+ \rightarrow [0,1]^{(Q \times Q) \times (Q \times Q)}$. For any $R \in \sigma^{-1}(P)$ we have that trivially 
+\begin{equation}\label{interchangeablerestandcomp}
+(\overline{\Psi} \circ \kappa_{r_k})_{|R} = \overline{\Psi}_{|R} \circ \kappa_{r_k}.
+\end{equation}
+Further, $((R, \Delta, \overline{\Psi}_{|R} \circ \kappa_{r_k}), \rho)$ is a Lyapunov system and recall that $S^1_R = ((R, \Sigma P, \overline{\Psi}_{|R}), (P, \Sigma P, \Psi'_{|P}), C^1_R)$ is a generalized Lyapunov system where $C^1_R = \{((q_1, q_2), q_2) \mid (q_1, q_2) \in R\}$. Let $V = \{q \in Q \mid (q, r_k) \in R\}$ and $\upsilon \in [0,1]^V$. Since $\supp(\upsilon \times e_{r_k}) \times \{r_k\} \in C^1_R$ by \Cref{from-gen-to-nongen} the limit $\lim_{n \rightarrow \infty} \frac1n \ln \|(\upsilon \times e_{r_k}) \overline{\Psi}_{|R}(w_n)\|$ exists $\PP_{e_{r_k}}$-almost surely and equals either $\lambda(S_R^1)$ or $-\infty$. Then, by (\ref{equalityofpushforward}) with $S = R$ we have for all $x \in [-\infty, 0]$ that 
+\begin{align}\label{equivofgeneralizedandnorm}
+& \PP_{e_{r_k}}(\{w \in (\Sigma Q)^\omega \mid \lim_{n \rightarrow \infty} \frac1n \ln \|(\upsilon \times e_{r_k}) \overline{\Psi}_{|R}(w_n)\| = x\}) \nonumber\\
+& = \PP_{\rho}(\{\overline{w} \in \Delta^\omega \mid \lim_{n \rightarrow \infty} \frac1n \ln \|(\upsilon \times e_{r_k}) \big[(\overline{\Psi}_{|R} \circ \kappa_{r_k})(\overline{w}_n)\big]\| = x\}).
+\end{align}
+Recall the definition of $\mathcal{L}$. The following series of equalities hold:
+\begin{equation}\label{possiblelyaplimits}
+\begin{aligned}
+& \lim_{n \rightarrow \infty} \frac1n \ln \|\mu_i \overline{\Psi}(w_n) \| \quad \PP_{e_{r_k}}\text{-a.s.}\\
+& = \lim_{n \rightarrow \infty} \frac1n \ln \|\mu_i \big[(\overline{\Psi} \circ \kappa_{r_k})(\overline{w}_n)\big] \| \quad \PP_{\rho}\text{-a.s.}  \quad \text{ by (\ref{equalityofpushforward}) where } S = Q \times Q\\ 
+& \in \Big\{\lambda((R, \Delta, (\overline{\Psi} \circ \kappa_{r_k})_{|R}), \rho) \mid R \in \mathcal{C} / \mathcal{L},  \supp~\mu_i \rightarrow_{G_{\mathcal{H}, \mathcal{H}}} R \Big\} \cup \{-\infty\} \, \PP_{\rho}\text{-a.s.} \\
+& \quad \quad \text{by \Cref{reduclyapsys}}\\
+& = \Big\{\lambda((R, \Delta, \overline{\Psi}_{|R} \circ \kappa_{r_k}), \rho) \mid R \in \sigma^{-1}(P) / \mathcal{L},  \supp~\mu_i \rightarrow_{G_{\mathcal{H}, \mathcal{H}}} R \Big\} \cup \{-\infty\} \\
+& \quad \quad \text{by (\ref{staysinP}) and (\ref{interchangeablerestandcomp})}\\ 
+& = \Big\{\lambda(\S_R^1) \mid R \in \sigma^{-1}(P) / \mathcal{L},  \supp~\mu_i \rightarrow_{G_{\mathcal{H}, \mathcal{H}}} R \Big\} \cup \{-\infty\} \quad \text{by (\ref{equivofgeneralizedandnorm})}.\\
+& = \Big\{\lambda(\S_R^1) \mid R \in \sigma^{-1}(P) /\mathcal{L},  \supp~\mu_i \rightarrow_{G_{\mathcal{H}, \mathcal{H}}} R \Big\} \cup \{-\infty\}.\\
+\end{aligned}
+\end{equation}
 
-
-Each limit   
-
-
-
-Write $H_{k,n}$
-
-
-
-
-
-%with prob 1 
-
-
-There is some word $w_k$ such that $\supp~ e_{(q, r)}\sum_{k = 1}^{n}\overline{\Psi}_{|R}(w_{k-1}) T(a_k r_k) \subset C$. Hence $\lim_{n \rightarrow \infty} \frac1n \ln \|\|$ 
-
-Clearly $\lim_{n \rightarrow \infty}\frac1n \ln \|\overline{\Psi}_{|C \cup R}(w_n)\| \geq \lim_{n \rightarrow \infty}\frac1n \ln \max \{ \|\overline{\Psi}_{|C}(w_n)\|, \|\overline{\Psi}_{|R}(w_n)\| \}$. Further, 
-
-
-Since $\|T\| \leq 1$ it follows that 
+We now focus on the case $i = 2$. Since $P$ is an SCC, there is a unique right-bottom SCC $P'$ that contains the states $\{(p, p) \mid p \in P\}$. Let $U'$ be another right-bottom SCC in the set $\sigma^{-1}(P) /\mathcal{L}$. Since $U'$ is an SCC and not in $\mathcal{L}$ we have that $\|\sum_{(s, r) \in U'}(e_s \times e_r)\overline{\Psi}_{|U'}(w_n)\| > 0$ for all $n \in \NN$. Therefore $\PP_{e_r}$-a.s. by \Cref{from-gen-to-nongen}, 
 \begin{align*}
-\lim_{n \rightarrow \infty}\frac1n \ln \| e_{(q, r)}\overline{\Psi}_{|C \cup R}(w_n)\| & = \lim_{n \rightarrow \infty}\frac1n \ln \Big[ \|e_{(q, r)} \sum_{k = 1}^{n} \overline{\Psi}_{|R}(w_{k-1}) T(a_k r_k)\overline{\Psi}_{|C}(w_{k+1,n}) \|\Big] \\
-& \leq \liminf_{n \rightarrow \infty} \max_{k \leq n} \frac1n \ln \Big[ \| e_{(q, r)} \overline{\Psi}_{|R}(w_{k-1}) T(a_k r_k) \overline{\Psi}_{|C}(w_{k+1,n}) \|\Big] \\
-& \leq \liminf_{n \rightarrow \infty} \frac1n \ln \Big[ \| e_{(q, r)} \overline{\Psi}_{|R}(w_{k_n-1}) T(a_{k_n} r_{k_n}) \overline{\Psi}_{|C}(w_{k_n+1,n}) \|\Big] \\
+\lambda(\S_{U'}^1) & = \lim_{n \rightarrow \infty} \frac1n \ln \|\sum_{(s, r) \in U'}(e_s \times e_r)\overline{\Psi}_{|U'}(w_n)\| \\
+& \leq \lim_{n \rightarrow \infty} \frac1n \ln |U'|\max_{(s, r) \in U'} \|(e_s \times e_r)\overline{\Psi}_{|U'}(w_n)\| \\
+& = \max_{(s, r) \in U'} \lim_{n \rightarrow \infty} \frac1n \ln \|(e_s \times e_r)\overline{\Psi}_{|U'}(w_n)\| \\
+& = \lambda(\S_{U'}^1) \text{ because each limit is either } \lambda(\S^1_{U'})\text{ or }-\infty 
 \end{align*}
-where $k_n(w) = \arg\max_{k \leq n} \frac1n \ln \| \overline{\Psi}_{|R}(a_1\cdots a_{k - 1}) T(a_k) \overline{\Psi}_{|C}(a_{k + 1} \cdots a_n) \|$. for $w \in \{n - k_n \rightarrow \infty\}$. 
+It follows that there is some $(s, r) \in U'$ such that $\PP_{e_r}(\lim_{n \rightarrow \infty} \frac1n \ln \|(e_s \times e_r)\overline{\Psi}_{|U'}(w_n)\| = \lambda(\S_{U'}^1)) > 0$.
+Let $U = \{q \in Q \mid \exists p\in Q \text{ s.t. }(q,p) \in U'\}$. Then $s \in U$, $r \in P$ and $(r, r) \in P'$. Hence, with $\PP_{e_r}$-probability greater than $0$ we have
+\begin{align*}
+0 & \geq \lim_{n \rightarrow \infty} \frac1n \ln \frac{\|e_s \Psi_{|U}(w_n)\|}{\|e_r \Psi_{|P}(w_n)\|} \text{ by \Cref{convergenceLn}}\\
+& = \lim_{n \rightarrow \infty} \frac1n \ln \frac{\|(e_s \times e_r) \overline{\Psi}_{|U'}(w_n)\|}{\|(e_r \times e_r) \overline{\Psi}_{|P'}(w_n)\|} \\
+& = \lim_{n \rightarrow \infty} \frac1n \big[ \ln \|(e_s \times e_r) \overline{\Psi}_{|U'}(w_n)\| - \ln \|(e_r \times e_r) \overline{\Psi}_{|P'}(w_n)\| \big] \\
+& = \lambda(\S_{U'}^1) - \lambda(\S_{P'}^1)
+\end{align*}
+which implies that $\lambda(\S^1_{P'}) \geq \lambda(\S^1_{U'})$. We have that $(r_k, r_k) \in \supp~ \mu_2$ and so $\PP_{e_{r_k}}$-almost surely we have ${\| (e_{r_k} \times e_{r_k}) \overline{\Psi}_{P'}(w_n) \| > 0}$ for all $n \in \NN$. By (\ref{staysinP}), it follows that $\PP_{e_{r_k}}$-a.s. we have
+\begin{align*}
+\lambda(\S_{P'}^1) & = \lim_{n \rightarrow \infty} \frac1n \ln \|(e_{r_k} \times e_{r_k}) \overline{\Psi}_{|P'}(w_n) \| \quad \text{ by \Cref{from-gen-to-nongen}}\\
+& \leq \lim_{n \rightarrow \infty} \frac1n \ln \|\mu_2 \overline{\Psi}(w_n) \|\\
+& \leq \max \Big\{\lambda(\S_R^1) \mid R \in \sigma^{-1}(P),~\supp~\mu_2 \rightarrow_{G_{\mathcal{H}, \mathcal{H}}} R \Big\} \text{ by (\ref{possiblelyaplimits})}\\
+& \leq \lambda(\S_{P'}^1).
+\end{align*}
+Then, recalling the definition of $S_R^2$ we have $\PP_{\pi_2}$-almost surely
+\begin{align*}\label{fixedutheoremversion}
+\lim_{n \rightarrow \infty} \frac{1}{k + n} \ln L_{k + n}(uw) & = \lim_{n \rightarrow \infty} \frac1n \Big[ \ln \| \mu_1 \overline{\Psi}(w_n) \| - \ln \|\mu_2 \overline{\Psi}(w_n) \| \Big] \nonumber\\
+& \in \Big\{\lambda(\S_R^1) - \lambda(S_{P'}^1) \mid R \in \sigma^{-1}(P), \supp~ \mu_1 \rightarrow_{G_{\mathcal{H}, \mathcal{H}}} R \Big\}\cup \{-\infty\} \\
+& = \Big\{\lambda(\S_R^1) - \lambda(S_R^2) \mid R \in \sigma^{-1}(P), \supp~ \mu_1 \rightarrow_{G_{\mathcal{H}, \mathcal{H}}} R \Big\}\cup \{-\infty\}
+\end{align*}
+since $\S_R^2 = \S_{P'}^1$ when $\sigma(R) = P$.
 
 
-Since $k_n \leq n$ we have that the sequence $k_n / n$ is bounded. Therefore by the Bolzano-Weierstrauss theorem there is a convergent subsequence $k_{a_n}$. 
+Recall that for any $R \in \mathcal{R}$ the right-bottom SCC $R'$ is such that $\{(p, p) \mid p \in \sigma(R)\} \subseteq R'$
 
-
-
-We have that $\supp~ e_i \overline{\Psi}_{|R}(w_{k_{a_n}-1})$ falls in a finite set, so without loss of generality we assume it is constant. 
-%We may assume that the subsequence also has the second part converging
-Hence, 
+We may now relax the dependence on $u$ and $P$. We have that $\supp~\pi_1 \times \supp~\pi_2 \rightarrow_{G_{\mathcal{H}, \mathcal{H}}} (\supp~ \pi_1 \Psi(a_1 \cdots a_k)) \times \{r_k\}$ for any $a_1 r_1 \cdots a_k r_k \in (\Sigma Q)^+$ where $\PP_{\pi_2}(Q a_1 r_1 \cdots a_k r_k (\Sigma Q)^\omega) > 0$. Therefore for all $R \in \mathcal{R}$ 
 \begin{equation*}
-\lim_{n \rightarrow \infty} \frac1n \ln \|\overline{\Psi}_{|C \cup R}(w_n)\| \in \{\lambda(\mathcal{S}^1_R) - \lambda(\mathcal{S}^2_R) \} \cup \{-\infty\} \cup \{\lambda(\mathcal{S}^1_{R'}) - \lambda(\mathcal{S}^2_{R'}) \mid R' \in \mathcal{R}, R' \subseteq C\}.
+(\supp~\pi_1 \Psi(a_1 \cdots a_k)) \times \{r_k\} \rightarrow_{G_{\mathcal{H}, \mathcal{H}}} R \implies  \supp~\pi_1 \times \supp~\pi_2 \rightarrow_{G_{\mathcal{H}, \mathcal{H}}} R.
 \end{equation*}
-Thus the claim holds for $C_{m+1} = C \cup R$. By induction the claim then holds for $C_M = C^*$ which completes the proof. 
+Finally we have up to a $\PP_{\pi_2}$-null set
+\begin{align*}
+& \{a_1 r_1 a_2 r_2 \cdots \in (\Sigma Q)^\omega \mid \exists k \in \NN \text{ s.t. } r_k \text{ is in a bottom SCC of } \mathcal{H}\} \\
+& \subseteq \Big\{\lim_{n \rightarrow \infty} \frac{1}{k + n} \ln L_{k + n}(uw) \\
+& \in \{-\infty\} \cup \big\{\lambda(\S_R^1) - \lambda(\S_R^2) \mid R \in \mathcal{R}, \supp~\pi_1 \times \supp~\pi_2 \rightarrow_{G_{\mathcal{H}, \mathcal{H}}} R \big\} \Big\}
+\end{align*}
+and the lemma follows.
 \end{proof}
 
 \section{Proofs from \cref{sec:det}} \label{app:det}

